Don't Forget to Buy Milk: Contextually Aware Grocery Reminder Household Robot

Assistive robots operating in household environments would require items to be available in the house to perform assistive tasks. However, when these items run out, the assistive robot must remind its user to buy the missing items. In this paper, we present a computational architecture that can allow a robot to learn personalized contextual knowledge of a household through interactions with its user. The architecture can then use the learned knowledge to make predictions about missing items from the household over a long period of time. The architecture integrates state-of-the-art perceptual learning algorithms, cognitive models of memory encoding and learning, a reasoning module for predicting missing items from the household, and a graphical user interface (GUI) to interact with the user. The architecture is integrated with the Fetch mobile manipulator robot and validated in a large indoor environment with multiple contexts and objects. Our experimental results show that the robot can adapt to an environment by learning contextual knowledge through interactions with its user. The robot can also use the learned knowledge to correctly predict missing items over multiple weeks and it is robust against sensory and perceptual errors.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\noindent Works related to grocery reminder systems are limited to ... Add papers from office desktop. 

Works on grocery related robots, on the hand, have focused on developing either grocery store robots that can navigate and assist people in finding groceries in the stores \cite{Dworakowski21}. OR robots that can deliver groceries MENTION. \cite{Liu21} grocery delivery algorithm optimization. \cite{chivarov21} service robot for transport and delivery of grocery products.
Grocery store robots? Not in homes.

Home service robots? Not for grocery reminders. Constrained?

Contextual understanding? 
Deep learning context learning? A lot of data, not personalized to the household.
